Analyzing Enterprise DNS Traffic to Classify Assets and Track Cyber-Health

The Domain Name System (DNS) is a critical service that enables domain names to be converted to IP addresses (or vice versa); consequently, it is generally permitted through enterprise security systems (e.g., firewalls) with little restriction. This has exposed organizational networks to DDoS, exfiltration, and reflection attacks, inflicting significant financial and reputational damage. Large organizations with loosely federated IT departments (e.g., Universities and Research Institutes) often do not even fully aware of all their DNS assets and vulnerabilities, let alone the attack surface they expose to the outside world. In this paper, we address the "DNS blind spot" by developing methods to passively analyze live DNS traffic, identify organizational DNS assets, and monitor their health on a continuous basis. Our contributions are threefold. First, we perform a comprehensive analysis of all DNS traffic in two large organizations (a University Campus and a Government Research Institute) for over a month, and identify key behavioral profiles for various asset types such as recursive resolvers, authoritative name servers, and mixed DNS servers. Second, we develop an unsupervised clustering method that classifies enterprise DNS assets using the behavioral attributes identified, and demonstrate that our method successfully classifies over 100 DNS assets across the two organizations. Third, our method continuously tracks various health metrics across the organizational DNS assets and identifies several instances of improper configuration, data exfiltration, DDoS, and reflection attacks. We believe the passive analysis methods in this paper can help enterprises monitor organizational DNS health in an automated and risk-free manner.

==> sections/perv/4traffichealth-VJ.tex <==
\section{Monitoring DNS Asset Health}\label{sec:health}
Having shown how DNS assets in an enterprise network can be identified and classified based on their network behavior, we now extend the study to monitor their health on a continuous basis. The objective is to detect \textit{anomalous} behavior, indicating that the asset is being misused or attacked, and identify the root cause of such deviations. We begin in \S\ref{sec:motivatingExample}
by providing two examples of observable anomalies from our dataset -- one attributable to poor configuration and the other subject to a DDoS attack. Inspired by these examples, in \S\ref{sec:metric} we suggest a set of \textit{health metrics} that can track the behaviour of each asset along various dimensions, and in \S\ref{sec:typeanomalies} develop a method to label and alert anomalous behaviors based on these continuous health tracking metrics. Finally in \S\ref{sec:insight} we apply our methods to the 32-day dataset from the two organisations, and prersent results into misuse and attack patterns detected by our methods.


\subsection{Examples Illustrating Anomalous DNS Asset Behavior}\label{sec:motivatingExample}
By manually inspecting our dataset, we could identify several behavioral patterns that seemed unusual. We therefore begin by providing a couple of illustrative examples of anomalous behavior (summarized in Table~\ref{tab:exampleHealth}), and subsequently develop methods to automatically detect these by tracking various health metrics.

\textbf{Example 1: DNS Misuse:} We found one of the Authoritative DNS Severs from the Research Institute dataset was responding with an unusually high number of ``{\myverb{NXDOMAIN}}'' messages. Upon investigation, we found that it was being queried with names that were irrelevant to the organisation, \eg ``{\myverb{www.taobao.com}}''. In fact 31.8\% of DNS queries to this server were irrelevant to the organisation, yet it was responding; a further 14.2\% were malformed (\eg ``{\myverb{com}}''), to which the server was responding with the ``{\myverb{NXDOMAIN}}'' message. This obviously represents a poorly configured server that is readily responding to every irrelevant and misformed query, rather than just the domains it is authoritative for, thereby opening up the server to a denial-of-service attack as well as a reflector for attacking others.

\textbf{Example 2: DNS Flood Attack:} We found one of the Authoritative DNS Servers in the University dataset to show a 142\% increase in inbound query rates over a 10-day period (7-Jun 0:17AM till 17-Jun 4:43PM). Upon closer inspection, we noted 3.3M queries, all with the same query name ``{\myverb{aids.gov}}'', had come during this period from 974 external sources -- typically each external source launched around 300 queries within a 20 second period, and then went idle. The DNS server was unable to keep up with the high rate of requests, and had a query service ratio of only about 70\%. Further, 40.9\% of the responses during this period were irrelevant to the organisation, while 21.6\% were with the ``{\myverb{NXDOMAIN}}'' error.


\subsection{DNS Traffic Health Metrics}\label{sec:metric}
Having seen some examples of poor behavior by DNS servers, we now propose several metrics that can be used to track the health of the DNS assets. We categorize them into service, functional, network, and volumetric profiles.

\textbf{Service profile:}
Authoritative name servers are expected to only service DNS queries seeking to resolve domains relevant to the enterprise. Conversely, recursive resolvers should only send outbound queries for domains outside of the enterprise. We therefore define {\myverb{Non-Enterprise Lookup Fraction (NELF)}} as the fraction of query names that are irrelevant to the enterprise services. A properly configured authoritative name server should have NELF of 0, while for a recursive resolver this should be 1.

\textbf{Functional profile:}
Under ideal conditions a properly functioning DNS server's response should always carry error code ``{\myverb{NoError}}'' -- occasional errors arise from typos which lead to non-existent names. We define a DNS server's {\myverb{Lookup Error Fraction (LEF)}} as the fraction of it's responses that carry an error code -- a value significantly larger than 0 indicates a potential mishbehavior.

\textbf{Network profile:}
Under normal circumstances a query is associated with a response. However, the network trace often reveals inbound responses with no outbound queries (e.g. a reflective attack to a victim whose IP address was spoofed), as well as outbound queries with no inbound response (e.g. a malicious internal host launching a DoS attack via the DNS cache/proxy). To track such anomalous network behavior, we define the Query Service Ratio, i.e. ratio of responses to queries, in the Inbound (QSRI) and Outbound (QSRO) directions. All DNS assets should ideally have these two metrics as 1, showing the balanced profile of queries and responses.

\textbf{Volumetric profile:}
Sudden increases in the rates of DNS packets can indicate that enterprise assets are being targeted by attacks. We therefore track the inbound and outbound rates of queries and responses for each DNS asset over each epoch (of one hour), respectively {\myverb{QryRateIn (QRI)}}, {\myverb{RespRateOut (RRO)}}, {\myverb{QryRateOut (QRO)}}, and {\myverb{RespRateIn (RRI)}}, and flag those epochs in which the rate shows an increase above a prescribed threshold value (discussed below), which could be indicative of volumetric attacks.


\subsection{Using Health Metrics to Detect Anomalies}\label{sec:typeanomalies}
The health metrics identified above can be used to detect and alert various anomalous behaviors of DNS assets. The set of anomalies we consider in this paper, illustrated in Fig.~\ref{fig:MappingAnomalyTypeTrafficHealth}, include:
\begin{temize}
\item {Misconfiguration:} Consider an Authoritative DNS Server that has been poorly configured, and resolves queries for domains that it has no authority over (i.e. do not belong to the enterprise). Exploitation of this by attackers (\eg as a reflector) will manifest in an alert for the NELF metric as being high, while LEF could also be high (in case the queries are malformed or non-existent). Conversely, for a poorly configured Recursive DNS Resolver, an alert is triggered when the NELF metric falls lower than a threshold.
\item {DDoS Attack:} A distributed denial-of-service attack on an enterprise DNS server will manifest in the form of a volumetric rise in QRI, potentially accompanied with a high NELF and/or LEF, since most queries in DDoS attacks tend to be either fixed or random rather than being crafted for the specific enterprise.
\item {Reflection Attack:} An inbound reflection attack on an enterprise asset usually targets the DNS cache/proxy, by bombarding it with unsolicited traffic. This will manifest in the form of a rising incoming response rate (RRI), as well as low ratio of outbound queries to incoming responses (QSRO).
\item {DNS Exfiltration:} An infected enterprise host that is trying to exfiltrate data via DNS will cause the QRO to rise, potentially accompanied with unanswered queries (rise in QSRO) and/or lookup errors (rise in LEF). These can be used as triggers to conduct deeper investigation into exfiltration, e.g. using our method in \cite{Jawad-TNSM20}.
\item {Scans:} Presence of malware that performs scans can be detected by monitoring for a rise in outbound queries (QRO), potentially accompanied with unanswered queries (rise in QSRO) and/or lookup errors (rise in LEF). 
\end{itemize}

In what follows we compute the health metrics of the various DNS assets in our dataset to identify anomalous behaviors as identified above.


\subsection{Evaluation in two Enterprise Networks}\label{sec:insight}
We applied the proposed traffic health metrics to our 32-day DNS traces captured from both organizations, comprising the assets as identified earlier in Tables~\ref{tab:clusterUNSW} and \ref{tab:clusterCSIRO} for the University and Research Institute respectively. The metrics are computed each epoch (lasting an hour), and we set up margin values for each of the health metrics to generate an alert indicating significant deviation from the expected values. The margin values were chosen as the elbow point in a curve representing the number of alerts generated for the chosen metric when plotted against the deviation threshold, ensuring that alerts were capturing deviations without being too frequent. This yielded a value of 30\%, whhich incidentally also corroborates with the threshold value used by many state-of-the-arts security middle-boxes from \cite{PaloAltoBestPractice2018}, Fortinet \cite{FortinetFirewallDDoS2018} and Cisco \cite{CISCOFirewallDDoS2018}. Organisations may tune the threshold values for each health metric to suit their environments. The health metric alerts are then fed into an inference engine that combines them to determine the nature of the anomaly, as discussed in \S\ref{sec:typeanomalies}. The health metric alerts, along with the underlying anomalies, are depicted in Table~\ref{tab:overviewHealth} for the assets in each of the two oganizations.

\subsubsection{Two Illustrative Examples}\label{sec:example}
Let us first examine two of DNS assets that exhibit the most anomalous behavior:

%129.94.31.47: woonona.austlii.unsw.edu.au: Australasian Legal Information Institute (AustLII), a joint facility of UTS and UNSW Faculties of Law.
\textbf{Example 1:}
A DNS server in the University Law Department serves as both authoritative name server and recursive resolver. It exhibited unhealthy elevated NELF metric for 83.7\% of epochs, and unhealthy depressed QSRI for 94.5\% of epochs, indicating its \textbf{misconfiguration} was being exploited by attackers for a potential \textbf{DDoS attack}. Queries for ``{\myverb{d.c.b.a.in-addr.arpa}}'' were coming from many external IP addresses, and the server was responding to a vast majority (over 90\%) of them, thereby wasting its resources. The asset also exhibited many epochs (6.6\%) of unhealthy LEF metric, indicating that it was proxying \textbf{scans}. On 29-Jun, this server sent queries to 131 external IP addresses, of which 18 responded -- this asset is likely being utilized as a proxy to perform slow reconnaissance scans to discover availability of DNS servers on the Internet as explored in detail in our other work \cite{MLyuTNSM2021}.

%For example, during 6:07AM on 29th June, this server sent 6 queries to an DNS resolver of Hurricane Electric LLC asking for non-existent domains with their patterns as {\myverb{*.hklii.org}}, where {\myverb{*}} is a random string.
%From 10:17AM to 10:19AM, 7 DNS queries with empty domain name {\myverb{nil}} were sent to a public resolver belonging to Amazon Technologies, which are replied with error code as {\myverb{Query Refused}}. 

%149.171.94.17: maestro.ee.unsw.edu.au:  
\textbf{Example 2:}
A DNS server in the University Engineering Department also exhibited many inbound health alerts, such as high NELP for 85.6\% of epochs, low QSRI for 15.6\% of epochs, and high QRI for 29.7\% of epochs. Investigation confirmed that it was \textbf{misconfigured} and exploited by attackers using it to launch reflection attacks with queries for domain names such as {\myverb{dnsscan.shadowserver.org}}, {\myverb{researchscan541.eecs.umich.edu}}, and {\myverb{nil}}. The sever was also giving outbound health alerts for high LEF, QSRO, and QRO, indicating potential for \textbf{DNS exfiltration}. Indeed, investigation showed that on 30-Jun it sent out 709K DNS queries with pattern {\myverb{SARICA[10digits].com}} towards an IP address in Turkey, and on the next day another 964K DNS queries to the same server with pattern {\myverb{akbank[9digits].com.tr}} - the random 9 or 10 digits very likely encode exfiltrated data \cite{JAhmedIM2019}.


\subsubsection{Enterprise-Wide Insights}\label{sec:summaryAlertStatistics}
Table~\ref{tab:overviewHealth} gives an overview of the alerts and anomalies for the assets in each of the two oganizations. While the number of alerts can is high, when combined to deduce anomalies they reveal that only a handful of DNS assets seem to be exposed to attacks. [Minzhao - I think we need to refine the table to show anomalies, not just alerts. For example, you can show how many of the authoritative name servers in each organisation seem to be misconfigured, how many are being used for scans, DDoS, reflections, etc.]

After presenting two examples to demonstrate how our metrics label unhealthy traffic status of DNS assets, we now discuss statistics of alerts for both organizations.

\textbf{Number of alerts on each asset:}
We show the number of alerts triggered by each monitored server per epoch as a CCDF plot in Fig.~\ref{fig:alertPerEpoch}.
It is clear that servers in the university are likely to have more alerts (\ie types of unhealthy DNS traffic) than their counterparts in the research institute.
Looking at the left side of both distributions in the figure (\ie $X = 0$), we can observe that about 40\% instances in the university campus do not have any alert, while the value for the research institute is much better (\ie 60\%).
As indicated by the right tails of the two distributions, there are two university DNS servers with 7 and 6 alert types during one epoch, which have already been discussed as example 1 and 2 in \S\ref{sec:example}. Besides, one asset in the research institute is with 5 alert types at one epoch -- its alert summary is shown as ``example 3'' in \S\ref{sec:example}.



\textbf{Temporal coverage of alerts by each asset:}
A DNS server would require more attention from operators if it keeps receiving alerts during its active time. We therefore quantify the alert temporal coverage of each server, which is shown as a CCDF plot in Fig.~\ref{fig:hostHealth}.
A server that continuously receives alert during all epochs has 1 in this value, while a server that has never been received any alert has 0 as its temporal coverage.
Surprisingly, no server had never received any alert during the 32 days, as all of them had been labeled unhealthy traffic alerts for inbound directions.
As shown by the two distributions in Fig.~\ref{fig:hostHealth}, DNS assets in the research institute have less alert temporal coverage than their counterparts in the university campus. 
Furthermore, 35\% and 13\% DNS servers in the university and research institute were consistently flagged by alerts -- all of them are configured by sub-departments and third-party entities.
Organizational recursive resolvers in both organizations have low temporal coverage of alerts, which are located in the top left corner of Fig.~\ref{fig:hostHealth} -- they only received {\myverb{high}} alerts in {\myverb{QryOut Increasing Rate}} and {\myverb{RespIn Increasing Rate}} during some epochs. 
%129.94.0.192 and 150.229.2.5
As the contrary, authoritative name servers were frequent targeted by inbound DNS attacks as they are more exposed to the public -- the primary organizational name servers in both networks have their alert temporal coverage as 67\% and 27\%, respectively.

\textbf{Comparison between the two organizations:}
We now compare the alerts in both networks, which is shown in the respective columns of Table~\ref{tab:overviewHealth}. Each cell contains the total counts and average temporal coverage of an alert type.
%
In the university network, DNS assets were often targeted by inbound non-enterprise and error lookups, given the high temporal coverage (35.5\% and 20.3\%) of  their respective alerts as highlighted by red cells in Table~\ref{tab:overviewHealth}.
In addition, {\myverb{high}} alerts in outbound error lookups are also worth noting for university servers.
As for the research institute, its DNS assets are heavily involved in outbound anomalies such as sending error lookups (on average 13.3\% alert temporal coverage), high outbound packet increasing rate for responses (12.0\%) and queries (11.9\%).
%
From the alert statistics above, we note that the university DNS assets are more frequently targeted by external attackers, while DNS servers in both organizations have non-negligible participation in anomalies toward external entities, especially through error lookups. 
Our study demonstrate the usefulness of our tools in locating insecure DNS assets in an enterprise network that are yet to be enforced via more effective security managements so that they will be more resistant to DNS-based cyber-crimes.



==> sections/perv/TitleAndAbstract.tex <==


\title{Analyzing Enterprise DNS Traffic to Classify Assets and Track Cyber-Health}

\IEEEtitleabstractindextext{%
	\begin{abstract}
		%word limit is 250 words
	
		The Domain Name System (DNS) is a critical service that enables domain names to be converted to IP addresses; consequently, it is generally permitted through enterprise security systems (\eg firewalls) without restriction. This has exposed organizational networks to DDoS, exfiltration, and reflection attacks, inflicting significant financial and reputational damage. Large organizations with loosely federated IT departments (\eg Universities and Research Institutes) often do not even know all their DNS assets, let alone the attack surface they expose to the outside world.

		In this paper we address the ``DNS blind spot'' by developing methods to passively analyze live DNS traffic, identify organizational DNS assets, and monitor their health on a continuous basis. Our first contribution performs a comprehensive analysis of all DNS traffic in two large organizations (a University Campus and a Government Research Institute) for over a month, and identifies key behavioral attributes for various asset types such as recursive resolvers, authoritative name servers, and mixed servers. For our second contribution we develop an unsupervised machine that classifies enterprise DNS assets using the behavioral attributes identified, and demonstrate that our method successfully identifies over a 100 DNS assets across the two organizations. Our final contribution continuously tracks various health metrics across the organizational DNS assets, and is able to identify several instances of improper configuration, data exfiltration, DDoS and reflection attacks. We believe the passive analysis methods in this paper can help enterprises monitor organizational DNS health in an automated and risk free manner.
	\end{abstract}
	
	\begin{IEEEkeywords}
		DNS forensics analysis, network security, enterprise host behavior.
	\end{IEEEkeywords}
}



==> sections/perv/intro-.tex <==
\vspace{7mm}
\IEEEraisesectionheading{\section{Introduction}\label{sec:intro}}
\IEEEPARstart{E}{nterprise} networks are not only large in size with many thousands of connected devices, but also dynamic in nature as hosts come and go, and servers get commissioned and decommissioned, to adapt to the organization's changing needs. Enterprise IT departments track such assets manually today, with records maintained in spreadsheets and configuration files (DHCP, DNS, Firewalls, etc.). This is not only cumbersome, but also error prone and almost impossible to keep up-to-date. It is therefore not surprising that many enterprise network administrators are not fully aware of their internal assets \cite{SMarshall2013}, and consequently do not know the attack surface they expose to the outside world.
The problem is even more acute in university and research institute campus networks for several reasons \cite{Deloitte2018}: (a) they host a wide variety of sensitive and lucrative data including intellectual property, cutting-edge research datasets, social security numbers, and financial information; (b) their open-access culture, decentralized departmental-level control, as well as federated access to data makes them particularly vulnerable targets for unauthorized access, unsafe Internet usage, and malware; and (c) they typically have high-speed network infrastructure that makes them an attractive target for volumetric reflection attacks.

DNS is one of the most favorite protocols exploited by cyber-crimes and botnets as it can easily bypass firewalls and security middleboxes. Due to DNS's nature of open-access, it is a common practice for organizations (\ie border firewalls) to apply little restrictions and monitoring of DNS traffic. 
Thus, it is unsurprising to see the increasing frequency and quantity of malware compromised devices and attacks that leverage DNS protocol \cite{EfficientIP2018,JVijayan2018,CFachkhaNTMS2014,US-CERT2018,MAnagnostopoulosCS2013}, such as DDoS attack, DNS tunneling and sensitive data exfiltration.

Enterprise hosts play different roles in DNS communications. 
An organizational network typically has a small number of recursive, caching resolvers that are configured to be used by internal hosts. 
Individual hosts may choose to manually change their preferred resolver to a public one (such as Google's public DNS resolvers at 8.8.8.8 and 8.8.4.4) but in general a majority of hosts will use a few caching servers for name resolution. 
Additionally, enterprises often have authoritative name servers for their organizational domains which can be distributed across departments depending on the size of the organization and the number of other public-facing servers (\eg organizational web-servers, data repositories or VPN services).
To secure their networks, it is important for organizational IT departments to understand and monitor DNS behaviors of connected hosts.

However, as reported in \cite{CiscoASR2016}, existing enterprise network security appliances such as border firewalls and intrusion detection systems do not provide a fine-grained visibility towards internal DNS related hosts and assets, leave it a `blind spot' for IT department.
Besides, although analysis of DNS traffic and DNS security are a hot topics in the research community, existing works either focused on forensic analysis of logs collected from DNS servers, such as recursive resolvers on the Internet \cite{XMATIFS2014,MAntonakakisSec2012,HGaoTNET2016,YChenDSN2014} and domain registrars \cite{SHaoCCS2016}, or concentrated on packet-level domain names \cite{YLeeCoNEXT2017,JAhmedIM2019,MAlmeidaCoNEXT2017,SSchuppenSec2018}. To the best of our knowledge, few prior work performed analysis on DNS traffic at enterprise network level to highlight potential DNS anomalies of an organization which is important to its security management.

In this paper\footnote{The detailed improvements from our prior work  \cite{MLyuPAM2019} are explained in \S\ref{sec:prior}.}, driven by the insights revealed by our forensic analysis of DNS traffic collected from edges of two representative enterprise networks, we develop an automatic method to map internal DNS Assets of an enterprise network using clustering algorithms, and track their DNS traffic health with well-articulated metrics that triggered alerts of various types each indicates a certain type of DNS anomaly.
%highlight on practical impact
The implemented system is deployed in the two enterprises. It lets administrators discover unknown assets configured by sub-departments, corroborate changes in host roles, understand potential vulnerabilities in their networks, and also equip them with information to configure appropriate security postures for their assets, such as to protect DNS resolvers from unsolicited responses, authoritative name servers from amplification requests, non-DNS servers from volumetric DNS reflection attacks, and block infected hosts generating unwanted DNS traffic.
Our specific contributions are summarized as three-fold.
 
\textbf{First}, in \S\ref{sec:analysis}, to understand the potential DNS threats faced by an enterprise, we performed a comprehensive forensic analysis of DNS traffic from two large organizations during 32 days, with highlights on their network, functional, and service properties.
We then highlight how DNS packet streams are differ amongst enterprise hosts playing different roles, with emphasis on their unique behavioral profiles that may exhibit suspicious patterns.

\textbf{Second}, in \S\ref{sec:class}, with the obtained knowledge, we identify key DNS traffic attributes of each enterprise host that can be extracted efficiently in real-time, and develop an unsupervised machine learning model using clustering algorithms to dynamically and continuously classify recursive resolvers, authoritative name-servers, dual-purpose DNS servers, and regular client hosts behind or not behind the NAT in an enterprise network.

\textbf{Third}, in \S\ref{sec:health}, driven by the fact that DNS anomalies (\eg attacks) cause deviation of asset traffic profiles, we develop monitoring metrics to track DNS traffic health of enterprise DNS asset and label types of unhealthy traffic patterns. Our practical method is applied to the 32-day DNS traffic traces of both organizations, which demonstrate it merits in enabling operators to locate, understand, and finally mitigate DNS threats within their networks.


%This paper is organized as follows.
%In \S\ref{sec:analysis} we analyze inbound and outbound DNS traffic of two enterprises at `network', `functional' and `service type' aspects, while revealing insights of unwanted packets in DNS traffic, and reveal host-level distribution of DNS queries and responses, with focus on composition of unwanted DNS traffic per enterprise host.
%In \S\ref{sec:class}, we identify important attributes of host DNS activity, describe our classification algorithm using the attributes and evaluate its results. 
%In \S\ref{sec:health}, we propose the metrics for monitoring DNS traffic health of enterprise DNS asset, and demonstrate its merits in inferring host anomalies.
Related works and our extension details are summarized in \S\ref{sec:prior}, and the paper is concluded in \S\ref{sec:concl}.



==> sections/perv/traffichealth-text.tex <==
\section{Monitoring Traffic Health of DNS Assets}\label{sec:health}
DNS assets in an enterprise network are vulnerable in various types of DNS anomalies such as being exploited to launch/reflect DNS attacks, hiding identity of attackers, or becoming victims of DNS cyber-crimes. 
The diverse types of DNS anomaly cause unusual deviations of asset DNS traffic profiles -- two examples and their impacts are discussed in \S\ref{sec:motivatingExample}.
To help IT departments locate, understand, and finally mitigate DNS security threats within their organizations, we develop a method of \textit{health metrics} to systematically monitor and track ``traffic health'' of each identified DNS asset (in \S\ref{sec:metric}). 
In \S\ref{sec:typeanomalies}, we describe how our method labels unhealthy DNS traffic profile through different alert types that reflect deviations of each health metric from its expected margin range.
We then apply the method of DNS traffic health tracking on our 32-day dataset and discuss insights into alerts from the two representative organizations (\S\ref{sec:insight}).  

\subsection{DNS Anomalies Causing Unhealthy Traffic Profiles}\label{sec:motivatingExample}
An enterprise asset may suffer from various types of DNS anomaly such as mis-configuration, under attacks, or mis-used as attack proxy, which inevitably cause its unhealthy DNS traffic profile (as discussed in \S\ref{sec:hostanalysis}).
We now present two examples of DNS anomaly identified in our dataset and highlight their impacts on traffic profiles of the corresponding assets, which is briefly summarized in Table~\ref{tab:exampleHealth}.

\textbf{Improper configuration:} 
An authoritative name server in the research institute is expected to only answer domain names belonging to the organization (\ie with the top-level domain as ``{\myverb{researchinstitute.com}}''). However, due to its improper configuration, this server sent responses for queries regardless their types and domains, which leads to unnecessary service exposure to malicious actors or mis-used as a recursive resolver.
As shown in the first row of Table~\ref{tab:exampleHealth}, 31.8\% of DNS lookups it responded were with ``{\myverb{NoError}}'' flags but their query names were irrelevant to the enterprise, such as ``{\myverb{www.taobao.com}}''.
In addition, 14.2\% of DNS lookups it responded were with errors, for example, this authoritative name server replied to a query for ``{\myverb{com}}'' with error ``{\myverb{NXDOMAIN}}''. 
Such occurrence of unhealthy DNS traffic could be avoided by configuring the server to only answer domain names it is authoritative for.

\textbf{Under a query flooding attack:}
A department authoritative name server in the university suffered from a 10-day query flooding attack since 0:17AM 7th June till 4:43PM 17th June.
Totally 3.3M queries (all with the same query name as ``{\myverb{aids.gov}}'') were sent to the server from 974 external attackers.
During the period, one attacker was active at the same time, which sent around 300 queries within 20 seconds and then went idle.
This victim server experienced high increasing rates of inbound queries (on average 142\%), and the ratio between inbound queries and outbound responses is 1.43 on average, far from the expected ratio value (\ie 1).
In addition, this server was also not properly configured and tried to answered all queries including the malicious ones, as the result, 21.6\% and 40.9\% of its answered questions are with errors and without error but irrelevant to the enterprise domain, respectively.

\subsection{Articulating Traffic Health Metrics}\label{sec:metric}

Now we describe our proposed health metrics of each identified DNS server inside an enterprise network, which track service, functional, network, and volumetric DNS traffic profiles of both inbound and outbound directions.

\textbf{Service profile:}
First, authoritative name servers are expected to only resolve DNS queries with its domain names relevant to an enterprise, while recursive resolvers should not send outbound queries asking for the enterprise domains.
We use {\myverb{non-Enterprise Lookup Fraction}} to describe the fraction of query names that are irrelevant to the enterprise services. 
Ideally, an authoritative name server answering lookups for enterprise domains are expect to have 0\% for this metric. Recursive resolvers that send outbound DNS queries are expected to have 100\% for this value.

\textbf{Functional profile:}
Second, a DNS server send responses with error code other than ``{\myverb{NoError}}'' to indicate that the requested domain names could not be answered correctly. Possible reasons include non-existent names, server failures, and others.
Thus, for each DNS asset, we define {\myverb{Error Lookup Fraction}} as the fraction of DNS lookups replied back with errors, which reflects the correctness of its DNS functionality.
A server with fully benign DNS traffic is expected to have 0 value for this metric.

\textbf{Network profile:}
Third, enterprise DNS assets may suffer from unanswered queries and unsolicited responses of both inbound and outbound directions. 
For example, an authoritative name server could become a victim in reflective DDoS attacks by receiving a massive amount of unsolicited inbound responses reflected by external resolvers; a recursive resolver may become a proxy that sends a large volume of malicious queries to external victims on behalf of an internal attacker.
To track unpaired lookups of each DNS asset, we come up with two metrics {\myverb{QryIn-RespOut Ratio}} and {\myverb{QryOut-RespIn Ratio}} to describe the quantity ratio between query and response of the two paired directions.
Ideally, all DNS assets should have the two metrics as 1, showing the balanced profile of queries and responses.

\textbf{Volumetric profile:}
Last, DNS attacks targeting or using enterprise assets may cause a sudden increase in traffic rate of DNS packets. 
We use the increasing rates of queries and responses from both directions to represent this traffic profile, namely {\myverb{QryIn Increasing Rate}}, {\myverb{RespOut Increasing Rate}}, {\myverb{QryOut Increasing Rate}}, and {\myverb{RespIn Increasing Rate}}.
The four metrics of each DNS server are expected to fall into an empirical range according to their normal activities. Out-of-range values of the increasing rates may indicate volumetric DNS anomalies on the asset.

\subsection{Labeling Alerts of Unhealthy DNS Traffic Patterns}\label{sec:typeanomalies}
Deviations of health metrics from its expected value range are indications of DNS anomalies (\eg under attacks) on a monitored DNS asset.
Our method labels alert type(s) of unhealthy DNS traffic according to the metrics that are deviated from its expected value ranges periodically.
Now we enumerate all alert types that could be raised for each metric respectively.

%type 1, irrelevant lookups fraction
First, considering the {\myverb{non-Enterprise Lookup Fraction}}, a {\myverb{high}} value alert will be raised for an authoritative name server answering too many queries that are irrelevant to the enterprise domains (\eg larger than 30\% of total fraction in our implementation); a recursive resolver will trigger a {\myverb{low}} value alert if it performs a large fraction of outbound lookups for enterprise domains (\eg less than 70\% for {\myverb{non-Enterprise Lookup Fraction}}).
%type 2,  error lookups fraction
Second, a DNS asset would be labeled with {\myverb{high}} value alerts if its {\myverb{Error Lookup Fraction}} is greater than a margin threshold defined by network operators (\eg 30\% in our implementation).
%type 3, query-response ratio
Third, a server would be labeled either with {\myverb{low}} or {\myverb{high}} value alerts for the two metrics {\myverb{QryOut-RespIn Ratio}} and {\myverb{QryIn-RespOut Ratio}} if their values fall out of a admin-defined range (\eg 0.7 to 1.3 in our setup).
%type 4, increasing rate
Last, the four metrics (\ie {\myverb{QryIn Increasing Rate}}, {\myverb{RespOut Increasing Rate}}, {\myverb{QryOut Increasing Rate}}, and {\myverb{RespIn Increasing Rate}}) monitor the increasing rate of inbound/outbound queries and responses, respectively.
If a metric is larger than the user-defined margin threshold (\eg 0.3), the asset would be labeled with {\myverb{high}} value alerts for its potential participation in DNS volumetric attacks.

Our metrics enable us to locate anomalous assets with unhealthy DNS traffic patterns due to various DNS anomaly types. In Fig.~\ref{fig:MappingAnomalyTypeTrafficHealth}, we visually show five example DNS anomaly types (while there are many other types that are not enumerated here) and the triggered unhealthy traffic alerts according to the evidences observed in our dataset.
For example, an authoritative name server may not be configured properly. As a consequence, it resolves queries (and performs recursive lookups) that do not contain top-level-domain names of the enterprise, which could lead to inbound and outbound alerts for the metrics of ``{\myverb{non-Enterprise Lookup Fraction}}'' and {\myverb{Error Lookup Fraction}} -- this mapping is clearly presented in Fig.~\ref{fig:MappingAnomalyTypeTrafficHealth}.


\subsection{Insights from two Enterprise Networks over 32 Days}\label{sec:insight}
We applied the proposed traffic health metrics to our 32-day DNS traces captured from both organizations.
Metrics for DNS assets in both enterprise networks (shown in Table~\ref{tab:clusterUNSW} and \ref{tab:clusterCSIRO}) were computed hourly, resulting in 39,687 and 27,135 instances\footnote{One instance contains the seven metrics and their corresponding alerts of a monitored DNS asset for each hour.} for the university and research institute respectively.

We set up margin values for health metrics that generate alerts to label their deviations in DNS traffic profiles. 
We conduct an empirical study on the two enterprises to decide a manageable value range in our implementation.
The elbow point is selected (\ie 0.3) as the margin value in our method. 
On average, IT departments of both organizations only have to focus on less than 15 DNS servers for further inspection per hour.
We note that a value around 0.3 is also a common margin value used by many state-of-the-arts security middle-boxes \cite{PaloAltoBestPractice2018,FortinetFirewallDDoS2018,CISCOFirewallDDoS2018}.
IT departments may select margin values using other strategies, such as a stricter range for certain prioritized metrics based on their needs.

In what follows, we reveal the insights into unhealthy DNS traffic from the two typical enterprises by analyzing alert statistics of two example DNS servers that are heavily involved in various types of anomalies (\S\ref{sec:example}), and overall alert statistics for the two enterprise networks (\S\ref{sec:summaryAlertStatistics}).
The alert types and their occurrences for the two example servers and the two enterprise networks are presented as the columns named ``Example 1'', ``Example 2'', ``University campus'', and ``Research institute'' in Table~\ref{tab:overviewHealth}, respectively.
For the two examples, each cell contains the total count of one alert type and its temporal coverage, for instance, the server ``Example 1'' was active for 768 monitoring epochs, and it received inbound alerts of {\myverb{high non-Enterprise Lookup Fraction}} during 643 epochs, thus, the temporal coverage of this alert for ``Example 1'' is 643/768 = 83.7\%.
As for the alert statistics of each organization, we show the total counts from all DNS assets and their average temporal coverage. 

\subsubsection{Two Illustrative Examples}\label{sec:example}
Now we discuss the two servers that are heavily suffered from unhealthy DNS traffic of both directions.

%129.94.31.47: woonona.austlii.unsw.edu.au: Australasian Legal Information Institute (AustLII), a joint facility of UTS and UNSW Faculties of Law.
\textbf{Example 1:}
%overview
The first example is a mixed DNS server operated by the university law department.
Over the 32 days, it heavily suffered from both inbound and outbound DNS anomalies.
%inbound
Considering the inbound alerts, this server received a large volume of anomalous queries, the majority of which are unanswered or answered but irrelevant to the enterprise domains.
As evidenced by the red cells under the column ``Example 1'' in Table~\ref{tab:overviewHealth}, the server triggered 643 {\myverb{high non-Enterprise Lookup Fraction}} and 726 {\myverb{high QryIn-RespOut Ratio}} alerts, covering 83.7\% and 94.5\% of its active duration, respectively.
We further look into the DNS traffic traces of this server, and identify that it is a frequent target of DNS query flooding attacks from distributed external hosts.
Those anomalous queries using question names that are mostly irrelevant to the enterprise, such as repeated reverse lookups ``{\myverb{d.c.b.a.in-addr.arpa}}'' for non-enterprise IP address ``{\myverb{a.b.c.d}}''. 
Surprisingly, a large amount of such queries (\ie more than 90\%) got responded by this server, showing its improper security configurations.
%outbound
As for its outbound alerts, it is clear that this department-level server consistently sent error lookups during its operating time.
Through an analysis of its DNS traffic traces, we found that the server periodically performed a small number of error DNS lookups toward a set of external DNS servers during the entire 32 days, which result in {\myverb{high}} alerts for outbound {\myverb{Error Lookup Fraction}}.
For example, during 6:07AM on 29th June, this server sent 6 queries to an DNS resolver of Hurricane Electric LLC asking for non-existent domains with their patterns as {\myverb{*.hklii.org}}, where {\myverb{*}} is a random string.
From 10:17AM to 10:19AM, 7 DNS queries with empty domain name {\myverb{nil}} were sent to a public resolver belonging to Amazon Technologies, which are replied with error code as {\myverb{Query Refused}}. 
On this day, such malicious queries were sent to a total of 131 external IP addresses, 18 of them replied back with errors while the rest 113 IPs did not send response -- this enterprise server is likely to be utilized as a proxy to perform slow reconnaissance scans \cite{MLyuTNSM2021} to discover availability of DNS servers on the Internet. 

%149.171.94.17: maestro.ee.unsw.edu.au:  
\textbf{Example 2:}
%overview
Similarly, a mixed DNS server hosted by the engineering department is also heavily involved in DNS anomalies of both directions, as highlighted by the red cells under the column ``Example 2'' in Table~\ref{tab:overviewHealth}.
%inbound
For the inbound alerts, the server triggered {\myverb{high non-Enterprise Lookup Fraction}} for its 85.6\% active duration due to a large amount of inbound queries with their domain names such as {\myverb{dnsscan.shadowserver.org}}, {\myverb{researchscan541.eecs.umich.edu}}, and {\myverb{nil}}.
Although the enterprise DNS server is not supposed to answer such irrelevant queries for external hosts, it still replied back with answers, which make it a valuable reflector and target in DNS cyber-crimes.
Unsurprisingly, due to the large amount of anomalies associated inbound queries, this server was also labeled with {\myverb{high}} alerts in {\myverb{QryIn-RespOut Ratio}} and {\myverb{QryIn Increasing Rate}} for 15.6\% and 29.7\% of its active duration.
%outbound
In Addition, this sever is also frequently involved in outbound DNS anomalies.
As shown by the high volume of alerts for {\myverb{high Error Lookup Fraction}}, {\myverb{high QryOut-RespIn Ratio}}, and {\myverb{high QryOut Increasing Ratio}} that covered 20.2\%, 84.4\%, and 31.1\% active time, this server sent out a large amount of outbound malicious queries that are unanswered or answered with errors.
Those abnormal outbound queries participated in various types of anomalous events such as volumetric attacks, scans, botnet controls, and data exfiltration.
For example, on 30th June, this server sent out 709K DNS queries with their names following the pattern of {\myverb{SARICA[10digits].com}} towards an IP address owned by Akbank in Turkey, where ``{\myverb{[10digits]}}'' is a 10-digit number looks randomly to the reader.
On next day, it sent 964K DNS queries to the same server with the name pattern as {\myverb{akbank[9digits].com.tr}}.
We note that all of them did not get any responses.
According to \cite{JAhmedIM2019}, such unusual activities are very likely to exfiltrate sensitive data from the organization to outside entities, the exfiltrated information is encoded as random digits in the domain names to bypass security detection.


\subsubsection{Alert Statistics of the Two Enterprises}\label{sec:summaryAlertStatistics}
After presenting two examples to demonstrate how our metrics label unhealthy traffic status of DNS assets, we now discuss statistics of alerts for both organizations.

\textbf{Number of alerts on each asset:}
We show the number of alerts triggered by each monitored server per epoch as a CCDF plot in Fig.~\ref{fig:alertPerEpoch}.
It is clear that servers in the university are likely to have more alerts (\ie types of unhealthy DNS traffic) than their counterparts in the research institute.
Looking at the left side of both distributions in the figure (\ie $X = 0$), we can observe that about 40\% instances in the university campus do not have any alert, while the value for the research institute is much better (\ie 60\%).
As indicated by the right tails of the two distributions, there are two university DNS servers with 7 and 6 alert types during one epoch, which have already been discussed as example 1 and 2 in \S\ref{sec:example}. Besides, one asset in the research institute is with 5 alert types at one epoch -- its alert summary is shown as ``example 3'' in \S\ref{sec:example}.



\textbf{Temporal coverage of alerts by each asset:}
A DNS server would require more attention from operators if it keeps receiving alerts during its active time. We therefore quantify the alert temporal coverage of each server, which is shown as a CCDF plot in Fig.~\ref{fig:hostHealth}.
A server that continuously receives alert during all epochs has 1 in this value, while a server that has never been received any alert has 0 as its temporal coverage.
Surprisingly, no server had never received any alert during the 32 days, as all of them had been labeled unhealthy traffic alerts for inbound directions.
As shown by the two distributions in Fig.~\ref{fig:hostHealth}, DNS assets in the research institute have less alert temporal coverage than their counterparts in the university campus. 
Furthermore, 35\% and 13\% DNS servers in the university and research institute were consistently flagged by alerts -- all of them are configured by sub-departments and third-party entities.
Organizational recursive resolvers in both organizations have low temporal coverage of alerts, which are located in the top left corner of Fig.~\ref{fig:hostHealth} -- they only received {\myverb{high}} alerts in {\myverb{QryOut Increasing Rate}} and {\myverb{RespIn Increasing Rate}} during some epochs. 
%129.94.0.192 and 150.229.2.5
As the contrary, authoritative name servers were frequent targeted by inbound DNS attacks as they are more exposed to the public -- the primary organizational name servers in both networks have their alert temporal coverage as 67\% and 27\%, respectively.

\textbf{Comparison between the two organizations:}
We now compare the alerts in both networks, which is shown in the respective columns of Table~\ref{tab:overviewHealth}. Each cell contains the total counts and average temporal coverage of an alert type.
%
In the university network, DNS assets were often targeted by inbound non-enterprise and error lookups, given the high temporal coverage (35.5\% and 20.3\%) of  their respective alerts as highlighted by red cells in Table~\ref{tab:overviewHealth}.
In addition, {\myverb{high}} alerts in outbound error lookups are also worth noting for university servers.
As for the research institute, its DNS assets are heavily involved in outbound anomalies such as sending error lookups (on average 13.3\% alert temporal coverage), high outbound packet increasing rate for responses (12.0\%) and queries (11.9\%).
%
From the alert statistics above, we note that the university DNS assets are more frequently targeted by external attackers, while DNS servers in both organizations have non-negligible participation in anomalies toward external entities, especially through error lookups. 
Our study demonstrate the usefulness of our tools in locating insecure DNS assets in an enterprise network that are yet to be enforced via more effective security managements so that they will be more resistant to DNS-based cyber-crimes.



==> sections/perv/traffichealth.tex <==
\begin{table*}[t!]
%	\vspace{-1mm}
	\caption{Example DNS anomalies and their impacts on traffic profiles.}
%	\vspace{-2mm}
	\centering
	\label{tab:exampleHealth}
	\begin{tabular}{|l|c|c|c|c|}
		\hline
		& \textbf{non-Enterprise Lookups} & \textbf{Error Lookups}    & \textbf{Qry Service Ratio} & \textbf{Qry Increasing Rate}  \\ \hline
		Improper configuration -- query resolving & {$\uparrow$} for inbound (31.8\%)    & {$\uparrow$} for inbound (14.2\%)  & -                   & -                   \\ \hline
		Under a 10-day query flooding attack          & {$\uparrow$} for inbound (40.9\%)  & {$\uparrow$} for inbound (21.6\%) & {$\uparrow$} for inbound (70\%)       & {$\uparrow$} for inbound (142\%)    \\ \hline
	\end{tabular}
%	\vspace{-6mm}
\end{table*}

\section{Monitoring DNS Asset Health}\label{sec:health}
Having shown how DNS assets in an enterprise network can be identified and classified based on their network behavior, we now extend the study to monitor their health on a continuous basis. The objective is to detect \textit{anomalous} behavior, indicating that the asset is being misused or attacked, and identify the root cause of such deviations. 
We begin in \S\ref{sec:motivatingExample} by providing two examples of observable anomalies from our dataset -- one attributable to poor configuration and the other subject to a DDoS attack. Inspired by these examples, in \S\ref{sec:metric} we suggest a set of \textit{health metrics} that can track the behavior of each asset along various dimensions, and in \S\ref{sec:typeanomalies} develop a method to label and alert anomalous behaviors based on these continuous health tracking metrics. Finally in \S\ref{sec:insight} we apply our methods to the 32-day dataset from the two organizations, and present results into misuse and attack patterns detected by our methods.


\subsection{Examples Illustrating Anomalous DNS Asset Behavior}\label{sec:motivatingExample}
By manually inspecting our dataset, we could identify several behavioral patterns that seemed unusual. We therefore begin by providing a couple of illustrative examples of anomalous behavior (summarized in Table~\ref{tab:exampleHealth}), and subsequently develop methods to automatically detect these by tracking various health metrics.

\textbf{Example 1 -- DNS Misuse:} We found one of the Authoritative DNS Severs from the Research Institute dataset was responding with an unusually high number of ``{\myverb{NXDOMAIN}}'' messages. Upon investigation, we found that it was being queried with names that were irrelevant to the organization, \eg ``{\myverb{www.taobao.com}}''. In fact 31.8\% of DNS queries to this server were irrelevant to the organization, yet it was responding; a further 14.2\% were malformed (\eg ``{\myverb{com}}''), to which the server was responding with the ``{\myverb{NXDOMAIN}}'' message. This obviously represents a poorly configured server that is readily responding to every irrelevant and malformed query, rather than just the domains it is authoritative for, thereby opening up the server to a denial-of-service attack as well as a reflector for attacking others.

\textbf{Example 2 -- DNS Flood Attack:} We found one of the Authoritative DNS Servers in the University dataset to show a 142\% increase in inbound query rates over a 10-day period (7-Jun 0:17AM till 17-Jun 4:43PM). Upon closer inspection, we noted 3.3M queries, all with the same query name ``{\myverb{aids.gov}}'', had come during this period from 974 external sources -- typically each external source launched around 300 queries within a 20 second period, and then went idle. The DNS server was unable to keep up with the high rate of requests, and had a query service ratio of only about 70\%. Further, 40.9\% of the responses during this period were irrelevant to the organization, while 21.6\% were with the ``{\myverb{NXDOMAIN}}'' error.

\subsection{DNS Traffic Health Metrics}\label{sec:metric}
Having seen some examples of poor behavior by DNS servers, we now propose several metrics that can be used to track the health of a DNS asset. We categorize them into service, functional, network, and volumetric profiles.

\textbf{Service profile:}
Authoritative name servers are expected to only serve DNS queries seeking to resolve domains relevant to the enterprise. Conversely, recursive resolvers should only send outbound queries for domains outside of the enterprise. We therefore define {\myverb{Non-Enterprise Lookup Fraction (NELF)}} as the fraction of query names that are irrelevant to the enterprise services. A properly configured authoritative name server should have {\myverb{NELF}} of 0, while for a recursive resolver this metric should be 1.

\textbf{Functional profile:}
Under ideal conditions a properly functioning DNS server's response should always carry error code ``{\myverb{NoError}}'' -- occasional errors arise from typos which lead to non-existent names. We define a DNS server's {\myverb{Lookup Error Fraction (LEF)}} as the fraction of it's responses that carry an error code -- a value significantly larger than 0 indicates a potential misbehavior.

\textbf{Network profile:}
Under normal circumstances a query is associated with a response. However, the network trace often reveals inbound responses with no outbound queries (\eg a reflective attack to a victim whose IP address was spoofed), as well as outbound queries with no inbound response (e.g. a malicious internal host launching a DoS attack via the DNS cache/proxy). To track such anomalous network behavior, we define the Query Service Ratio, i.e. ratio of responses to queries, in the Inbound (QSRI) and Outbound (QSRO) directions. All DNS assets should ideally have these two metrics as 1, showing the balanced profile of queries and responses.

\textbf{Volumetric profile:}
Sudden increases in the rates of DNS packets can indicate that enterprise assets are being targeted by attacks. We therefore track the inbound and outbound rates of queries and responses for each DNS asset over each epoch (of one hour), respectively {\myverb{QryRateIn (QRI)}}, {\myverb{RespRateOut (RRO)}}, {\myverb{QryRateOut (QRO)}}, and {\myverb{RespRateIn (RRI)}}, and flag those epochs in which the rate shows an increase above a prescribed threshold value (discussed below), which could be indicative of volumetric attacks.


\begin{figure}[t!]
%	\vspace{-1mm}
	\begin{center}
		{\includegraphics[width=0.5\textwidth]{fig/AnomalyAndTraffic.pdf}}
	%	\vspace{-2mm}
		\caption{Some examples of our observed DNS anomalies and their related traffic health alerts.}
		%		\vspace{-4mm}
		\label{fig:MappingAnomalyTypeTrafficHealth}
	\end{center}
%	\vspace{-9mm}
\end{figure}

\subsection{Using Health Metrics to Detect Anomalies}\label{sec:typeanomalies}
The health metrics identified above can be used to detect and alert various anomalous behaviors of DNS assets. The set of anomalies we consider in this paper, illustrated in Fig.~\ref{fig:MappingAnomalyTypeTrafficHealth}, include:
\begin{itemize}
	\item {\textbf{Misconfiguration:}} Consider an Authoritative DNS Server that has been poorly configured, and resolves queries for domains that it has no authority over (i.e. do not belong to the enterprise). Exploitation of this by attackers (\eg as a reflector) will manifest in an alert for the NELF metric as being high, while LEF could also be high (in case the queries are malformed or non-existent). Conversely, for a poorly configured Recursive DNS Resolver, an alert is triggered when the NELF metric falls lower than a threshold.
	\item {\textbf{DDoS Attack:}} A distributed denial-of-service attack on an enterprise DNS server will manifest in the form of a volumetric rise in QRI, potentially accompanied with a high NELF and/or LEF, since most queries in DDoS attacks tend to be either fixed or random rather than being crafted for the specific enterprise.
	\item {\textbf{Reflection Attack:}} An inbound reflection attack on an enterprise asset usually targets the DNS cache/proxy, by bombarding it with unsolicited traffic. This will manifest in the form of a rising incoming response rate (RRI), as well as low ratio of outbound queries to incoming responses (QSRO).
	\item {\textbf{DNS Exfiltration:}} An infected enterprise host that is trying to exfiltrate data via DNS will cause the QRO to rise, potentially accompanied with unanswered queries (rise in QSRO) and/or lookup errors (rise in LEF). These can be used as triggers to conduct deeper investigation into exfiltration, e.g. using the method in \cite{JAhmedTNSM2020}.
	\item {\textbf{Scans:}} Presence of malware that performs scans can be detected by monitoring for a rise in outbound queries (QRO), potentially accompanied with unanswered queries (rise in QSRO) and/or lookup errors (rise in LEF). 
\end{itemize}

In what follows we compute the health metrics of the various DNS assets in our dataset to identify anomalous behaviors that causes unusual changes of our metrics as some examples listed above.

\begin{table}[t!]
%	\vspace{-3mm}
	\caption{Alerts and their occurrence for our three examples over 32 days.}
	\centering
	\label{tab:exampleAlert}
%	\vspace{-2mm}
	\begin{tabular}{|c|c|c|cc|}
		\hline
	\textbf{Direct.}& \textbf{Profile}&	\textbf{Alert}   &  \textbf{Example 1}& \textbf{Example 2}  \\ \hline\hline
		In.&Service&high NELF   &\cellcolor{red!25} 643 (83.7\%) & \cellcolor{red!25}636 (85.6\%)  \\ \hline
		In.&Functional&	high LEF     & 51 (6.6\%) &5 (0.1\%)    \\ \hline
		In.&Network&	low QSRI     &  \cellcolor{red!25}726 (94.5\%) & \cellcolor{red!25}116 (15.6\%)  \\ \hline
		In.&Network&	high QSRO    & 1 (0.1\%) & 2 (0.3\%) \\ \hline
		In.&Volmetric&	high QRI& 0 (0.0\%) & \cellcolor{red!25}221 (29.7\%) \\ \hline
		In.&Volmetric&	high RRI & 39 (5.1\%)  &73 (9.8\%)  \\ \hline\hline
		
		Out.&Service&	low NELF & 0 (0.0\%) &0 (0.0\%) \\ \hline	
		Out.&Functional&high LEF & \cellcolor{red!25} 768 (100.0\%)  & \cellcolor{red!25}150 (20.2\%)\\ \hline
		Out.&Network&	high QSRI      &  6 (0.8\%) &2 (0.3\%)\\ \hline
		Out.&Network&	low QSRO    &  0 (0.0\%)  &\cellcolor{red!25}627 (84.4\%) \\ \hline	
		Out.&Volumetric&	high RRO  & 43 (5.6\%) &57 (7.7\%)\\ \hline
		Out.&Volumetric&	high QRO & 8 (1.0\%) & \cellcolor{red!25}231 (31.1\%)\\ \hline	
	\end{tabular}
%	\vspace{-5mm}
\end{table}


\begin{figure}[t!]
	%	\vspace{-1mm}
	\begin{center}
		{\includegraphics[width=0.4\textwidth]{fig/CCDF/ccdfHostHealth.pdf}}
		%	\vspace{-2mm}
		\caption{Temporal coverage of alerts per server.}
		%		\vspace{-4mm}
		\label{fig:hostHealth}
	\end{center}
	%	\vspace{-9mm}
\end{figure}

\subsection{Insights in two Enterprise Networks}\label{sec:insight}
We applied the proposed traffic health metrics to our 32-day DNS traces captured from both organizations, comprising the assets as identified earlier in Tables~\ref{tab:clusterUNSW} and \ref{tab:clusterCSIRO} for the University (67 DNS servers) and Research Institute (40 DNS servers) respectively. 
The metrics are computed each epoch (lasting an hour), and we set up margin values for each of the health metrics to generate an alert indicating significant deviation from the expected values. 
The margin values were chosen as the elbow point in a curve representing the number of alerts generated for the chosen metric when plotted against the deviation threshold, ensuring that alerts were capturing deviations without being too frequent. This yielded a value of 30\%, which incidentally also corroborates with the threshold value used by many state-of-the-arts security middle-boxes from Palo Alto \cite{PaloAltoBestPractice2018}, Fortinet \cite{FortinetFirewallDDoS2018} and Cisco \cite{CISCOFirewallDDoS2018}. 
Organizations may tune the threshold values for each health metric to suit their environments. 
The health metric alerts are then fed into an inference engine that combines them and performs necessary further investigation to determine the nature of the anomaly, as discussed in \S\ref{sec:typeanomalies}. 

\subsubsection{Two Illustrative Examples}\label{sec:example}
Let us first examine two of DNS assets that exhibit the most anomalous behavior, the alerts of which are shown in Table~\ref{tab:exampleAlert}:

%129.94.31.47: woonona.austlii.unsw.edu.au: Australasian Legal Information Institute (AustLII), a joint facility of UTS and UNSW Faculties of Law.
\textbf{Example 1:}
A DNS server in the University Law Department serves as both authoritative name server and recursive resolver. It exhibited unhealthy elevated NELF metric for 83.7\% of epochs, and unhealthy depressed QSRI for 94.5\% of epochs, indicating its \textbf{misconfiguration} was being exploited by attackers for a potential \textbf{DDoS attack}. Queries for ``{\myverb{d.c.b.a.in-addr.arpa}}'' were coming from many external IP addresses, and the server was responding to a vast majority (over 90\%) of them, thereby wasting its resources. The asset also exhibited many epochs (6.6\%) of unhealthy LEF metric, indicating that it was proxying \textbf{scans}. On 29-Jun, this server sent queries to 131 external IP addresses, of which 18 responded -- this asset is likely being utilized as a proxy to perform slow reconnaissance scans to discover availability of DNS servers on the Internet as explored in detail in our other work \cite{MLyuTNSM2021}.

%149.171.94.17: maestro.ee.unsw.edu.au:  
\textbf{Example 2:}
A DNS server in the University Engineering Department also exhibited many inbound health alerts, such as high NELP for 85.6\% of epochs, low QSRI for 15.6\% of epochs, and high QRI for 29.7\% of epochs. Investigation confirmed that it was \textbf{misconfigured} and exploited by attackers using it to launch reflection attacks with queries for domain names such as {\myverb{dnsscan.shadowserver.org}}, {\myverb{researchscan541.eecs.umich.edu}}, and {\myverb{nil}}. The sever was also giving outbound health alerts for high LEF, QSRO, and QRO, indicating potential for \textbf{DNS exfiltration}. Indeed, investigation showed that on 30-Jun it sent out 709K DNS queries with pattern {\myverb{SARICA[10digits].com}} towards an IP address in Turkey, and on the next day another 964K DNS queries to the same server with pattern {\myverb{akbank[9digits].com.tr}} - the random 9 or 10 digits very likely encode exfiltrated data as highlighted in \cite{JAhmedTNSM2020}.

\begin{table*}[t!]
	\caption{DNS anomalies on enterprise assets and their occurrences in both organizations.}
	\centering
	\label{tab:InferDNSAnomalies}
	%66 Uni 40 Research
%	\hspace{-4mm}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
	\textbf{ DNS Anomaly}&	\textbf{Indicative Alerts}   & \textbf{Post-hoc Analysis} & \textbf{\textbf{{\color{red}High}:{\color{orange}Medium}:{\color{yellow}Low}:{\color{green}None}} -- Univ.} & \textbf{\textbf{{\color{red}High}:{\color{orange}Medium}:{\color{yellow}Low}:{\color{green}None}} -- Rsrch.}  \\ \hline\hline
	Misconfiguration & $\uparrow$ NELF \& LEF & None &\textbf{{\color{red}38(56\%)}:{\color{orange}2(3\%)}:{\color{yellow}5(7\%)}:{\color{green}22(33\%)}}  & \textbf{{\color{red}13(33\%)}:{\color{orange}0(0\%)}:{\color{yellow}11(28\%)}:{\color{green}24(60\%)}}   \\ \hline
	Query-based DDoS & $\uparrow$ QSRI \& QRI & Flow profile &\textbf{{\color{red}1(1\%)}:{\color{orange}0(\%)}:{\color{yellow}12(18\%)}:{\color{green}54(80\%)}}  & \textbf{{\color{red}0(0\%)}:{\color{orange}0(0\%)}:{\color{yellow}4(10\%)}:{\color{green}36(90\%)}}  \\ \hline
	Resp.-based DDoS & $\downarrow$ QSRO \& $\uparrow$ RRI & Flow profile &\textbf{{\color{red}1(1\%)}:{\color{orange}1(1\%)}:{\color{yellow}7(10\%)}:{\color{green}58(87\%)}}& \textbf{{\color{red}0(0\%)}:{\color{orange}0(0\%)}:{\color{yellow}12(30\%)}:{\color{green}28(70\%)}} \\ \hline
	Reflectors in attacks & $\uparrow$  QRI \& RRO & Flow profile &\textbf{{\color{red}17(25\%)}:{\color{orange}4(6\%)}:{\color{yellow}7(10\%)}:{\color{green}39(58\%)}} & \textbf{{\color{red}8(20\%)}:{\color{orange}0(0\%)}:{\color{yellow}7(18\%)}:{\color{green}25(63\%)}} \\ \hline
	Generating scans & $\uparrow$ LEF \& $\downarrow$ QSRO & Flow profile& \textbf{{\color{red}3(4\%)}:{\color{orange}4(6\%)}:{\color{yellow}10(15\%)}:{\color{green}50(75\%)}}&  \textbf{{\color{red}2(5\%)}:{\color{orange}4(10\%)}:{\color{yellow}10(25\%)}:{\color{green}24(60\%)}} \\ \hline
	Data exfiltrations & $\uparrow$ LEF \& QRO  \& $\downarrow$ QSRO&  Query content & \textbf{{\color{red}0(0\%)}:{\color{orange}0(0\%)}:{\color{yellow}8(12\%)}:{\color{green}59(88\%)}}  &  \textbf{{\color{red}0(0\%)}:{\color{orange}0(0\%)}:{\color{yellow}5(13\%)}:{\color{green}35(88\%)}}  \\ \hline
	
Reflectors after config.& $\uparrow$ QRI \& RRO &Flow profile& \textbf{{\color{red}2(3\%)}:{\color{orange}1(1\%)}:{\color{yellow}8(12\%)}:{\color{green}56(84\%)}} & \textbf{{\color{red}0(0\%)}:{\color{orange}0(0\%)}:{\color{yellow}4(10\%)}:{\color{green}36(90\%)}} \\ \hline
	
	\end{tabular}
\end{table*}

\subsubsection{Analyzing Alert Statistics of the Two Enterprises}\label{sec:summaryAlertStatistics}
After presenting two examples to demonstrate how our metrics label unhealthy traffic status of DNS assets, we now analyze statistics of alerts in both organizations.

\textbf{Temporal coverage of alerts by each asset:}
A DNS server would require more attention from operators if it keeps receiving alerts during its active time. We therefore quantify the alert temporal coverage of each server, which is shown as a CCDF plot in Fig.~\ref{fig:hostHealth}.
A server that continuously receives alert during all epochs has 1 in this value, while a server that has never been received any alert has 0 as its temporal coverage.
Surprisingly, no server had never received any alert during the 32 days, as all of them had been labeled unhealthy traffic alerts for inbound directions.
As shown by the two distributions in Fig.~\ref{fig:hostHealth}, DNS assets in the research institute have less alert temporal coverage than their counterparts in the university campus. 
Furthermore, 35\% and 13\% DNS servers in the university and research institute were consistently flagged by alerts -- all of them are configured by sub-departments and third-party entities.
Organizational recursive resolvers in both organizations have low temporal coverage of alerts, which are located in the top left corner of Fig.~\ref{fig:hostHealth} -- they only received {\myverb{high}} alerts in {\myverb{QryOut Increasing Rate}} and {\myverb{RespIn Increasing Rate}} during some epochs. 
%129.94.0.192 and 150.229.2.5
As the contrary, authoritative name servers were frequent targeted by inbound DNS attacks as they are more exposed to the public -- the primary organizational name servers in both networks have their alert temporal coverage as 67\% and 27\%, respectively.

{\color{blue}
\textbf{Inferring asset DNS anomalies from alerts:}
Just as doctors diagnose diseases from observations of symptoms, we are able to infer DNS anomaly types by collectively considering traffic health alerts of each asset with necessary post-hoc forensics analysis (some examples have been discussed in \S\ref{sec:example}).
We now present the number of assets confirmed with 6 example DNS anomalies considered in this paper (as already shown in Fig.~\ref{fig:MappingAnomalyTypeTrafficHealth}) from our 32-day dataset. 
As shown in the top six rows of Table~\ref{tab:InferDNSAnomalies}, for each DNS anomaly type in both enterprises, we list the indicative alerts that triggers post-hoc forensics analysis, the number and fraction of confirmed assets with high (\ie more than 66\% of epochs), medium (\ie 33\% to 66\% of epochs), low (\ie less than 33\% of epochs), and none occurrence of the anomaly.
%1. majority of asset are healtthy
We can observe that for all types of anomalies (except misconfiguration in the university network), more than 50\% of DNS assets in both organizations are healthy, as shown by the ``None'' occurrence values marked by green color.
%2. the major problem -- misconfig.
It is also clear that misconfiguration is the predominant problem in both networks -- 56\% and 33\% DNS servers are with high occurrence in the university and research institute, respectively.
%3.the lightest problem in univ. and rsrch.
In the university network, data exfiltration via DNS query names is the most infrequent problem with only 12\% assets marked by ``low'' occurrence, and misused as reflectors in DDoS attacks in the lightest one in the research institute, with only 10\% DNS assets under the ``low'' occurrence category.

%4.mitigating misconfiguration
With the obtained knowledge of identified DNS assets and their anomalies inferred by our metrics, IT departments could enforce their security management through various measures, such as not allowing inbound DNS queries toward internal recursive resolvers on the border firewall, operating recursive resolver and authoritative name servers on separate IP addresses, and rate-limiting lookups performed for each external IP addresses to reduce their capability in reflecting attacks.
Let's take the misconfiguration problem as an example. We perform a simulation on our dataset to demonstrate the scenario if all DNS assets are securely configured for query resolving -- authoritative name servers only respond to queries contains top-level domains of the enterprise and recursive resolvers do not perform lookups for external IP addresses.
From our result, we conclude that applying the security policies not only solve the misconfiguration problem (by reducing the number of occurrence to 0), but also alleviate other anomaly types. 
As shown in the last row of Table~\ref{tab:InferDNSAnomalies}, the fraction of benign assets for 'misused as reflectors in attacks' increases from 58\% to 84\% in the university and from 63\% to 90\% in the research institute, moreover, the DNS assets that are highly affected by this anomaly drops significantly from 25\% to 3\% and 20\% to 0\% in the two networks.
Undoubtedly, our method that identifies and tracks DNS assets within an enterprise is utmost helpful for IT departments to make proper and precise DNS security enforcement to effectively and securely management their networks.
}


